Auditable Algebraic Counting Field for Cryptic-Pocket Detection from Apo Structures

Cryptic ligand-binding pockets are not apparent in experimentally determined apo structures, making them difficult to identify from unbound receptor geometry. A complementary challenge is to make the structural measurements and learned evidence behind each prediction directly inspectable. We introduce a supervised algebraic counting field (ACF) for predicting cryptic-pocket residues from apo structures. ACF compiles explicit geometric, physicochemical, and topological features into compact, integer-weighted lookup tables. Each prediction score can be reconstructed from feature values, training counts, table weights, and spatial aggregation, without sequence search, structural-template transfer, or a protein language model at inference. We evaluate ACF on CryptoBench and two locked external collections, separating ranking performance from the effects of residue-calling budgets. On an external set of 57 post-CryptoBench apo-holo units, ACF exceeded P2Rank by +0.044 in mean paired ROC-AUC (multiplicity-adjusted 95% CI [+0.010, +0.079]). The advantage was dataset-dependent: official-fold ROC-AUC and matched-budget F1 differences against P2Rank remained unresolved, and a second external evaluation did not confirm gains from added structural features. ACF thus provides a compact predictor with externally validated signal and an inspectable path from structural measurements and training counts to residue scores.

==> generated_case_table.tex <==
\begin{table}[t]
\tbl{Post hoc descriptive extremes of the per-structure F1 difference. These cases illustrate heterogeneity and are not a confirmatory subset.}
{\begin{tabular}{@{}lrrrr@{}}
\toprule
Unit & True residues & Field F1 & P2Rank F1 & Difference\\
\midrule
6bty\_B & 9 & 0.095 & 0.571 & -0.476\\
3idh\_A & 22 & 0.000 & 0.386 & -0.386\\
5e0v\_A & 15 & 0.162 & 0.545 & -0.383\\
2d05\_A & 22 & 0.889 & 0.293 & +0.596\\
4p2f\_A & 10 & 0.519 & 0.000 & +0.519\\
2vl2\_C & 10 & 0.417 & 0.000 & +0.417\\
\bottomrule
\end{tabular}}
\label{tab:case-extremes}
\end{table}

